Deep Affinity Net: Instance Segmentation via Affinity

Most of the modern instance segmentation approaches fall into two categories: region-based approaches in which object bounding boxes are detected first and later used in cropping and segmenting instances; and keypoint-based approaches in which individual instances are represented by a set of keypoints followed by a dense pixel clustering around those keypoints. Despite the maturity of these two paradigms, we would like to report an alternative affinity-based paradigm where instances are segmented based on densely predicted affinities and graph partitioning algorithms. Such affinity-based approaches indicate that high-level graph features other than regions or keypoints can be directly applied in the instance segmentation task. In this work, we propose Deep Affinity Net, an effective affinity-based approach accompanied with a new graph partitioning algorithm Cascade-GAEC. Without bells and whistles, our end-to-end model results in 32.4% AP on Cityscapes val and 27.5% AP on test. It achieves the best single-shot result as well as the fastest running time among all affinity-based models. It also outperforms the region-based method Mask R-CNN.

==> TEX/title.tex <==
%\title{AgImageNet: Visual Recognition Challenges for Agricultural Aerial Images and A New Benchmark}
\title{Deep Affinity Net: Instance Segmentation via Pixel Affinity}

\author{
Xingqian Xu\\
Beckman Institute, UIUC\\
{\tt\small xu16@illinois.edu}
% % For a paper whose authors are all at the same institution,
% % omit the following lines up until the closing ``}''.
% % Additional authors and addresses can be added with ``\and'',
% % just like the second author.
% % To save space, use either the email address or home page, not both
\and
MangTik Chiu\\
Beckman Institute, UIUC\\
{\tt\small mtchiu2@illinois.edu}
\and
Honghui Shi\\
Beckman Institute, UIUC\\
{\tt\small hshi10@illinois.edu}
\and
Thomas S. Huang\\
Beckman Institute, UIUC\\
{\tt\small t-huang1@illinois.edu}
}

\maketitle
% %\thispagestyle{empty}
